NoMAD-Attention: Efficient LLM Inference on CPUs Through Multiply-add-free Attention

Large language model inference on Central Processing Units (CPU) is challenging due to the vast quantities of expensive Multiply-Add (MAD) matrix operations in the attention computations. In this paper, we argue that there is a rare gem in modern CPUs, Single-Instruction-Multiple-Data (SIMD) registers, which allow for ultra-low-latency lookups in batch. We leverage this unique capability of CPUs to propose NoMAD-Attention, an efficient attention algorithm that replaces MAD operations with in-register lookups. Through hardware-aware algorithmic designs, NoMAD-Attention achieves the computation of attention scores using repeated fast accesses to SIMD registers despite their highly limited sizes. Moreover, NoMAD-Attention works with pre-trained attention-based LLMs without model finetuning. Empirical evaluations demonstrate that NoMAD-Attention maintains the quality of the original LLMs well, and speeds up the 4-bit quantized LLaMA-7B-based model by up to 2$\times$ at 16k context length. Our results are reproducible at https://github.com/tonyzhang617/nomad-dist.

==> icml2024/trash/archive.tex <==

In the decoding phase, the embedding of the current token passes through a sequence of multi-layer perceptrons (MLP), attention, and normalization layers. Only the attention layers model the interaction between the current token and other tokens, the other components of an LLM performs transformations based on the embedding of the current token with no dependence on other tokens. Therefore, for the $t$-th decoding step, the time complexity of attention is $O(t)$ while the time complexity of other layers is $O(1)$. By improving the efficiency of attention score computations, the bottleneck of LLM inference can be mitigated, especially for longer sequence length.

% We will refer to the results of $\mathrm{softmax}(\frac{qK^\top}{\sqrt d})$ as attention scores, which dictate how much attention each token pays to all other tokens. 


\subsection{KV Caching Technique}

Key-value (KV) caching is a technique employed to enhance the efficiency of the inference process in autoregressive large language models (LLMs) such as GPT, T5, and Llama. In autoregressive models, tokens are generated sequentially until predefined stopping criteria are met, such as reaching the specified maximum sequence length or generating a stop sequence like a single end-of-sequence (EOS) token. This sequential token generation incurs a substantial computational burden due to the recomputation of attention values within the key ($K$) and value ($V$) matrices. To mitigate this overhead, KV caching operates by storing previously computed Key-Value matrices, representing tokens from the generated text to reduce the repetitive computation.

The autoregressive generation typically involves two distinct phases: (i) the \textbf{initialization} (or \textbf{prefill}) phase begins with a prompt sequence, leading to the generation of the KV cache for each transformer layer within the LLM, and (ii) the \textbf{generation} (or \textbf{decode}) phase leverages and updates the KV cache to generate tokens incrementally. \cite{sheng2023flexgen}

For a specific LLM generative inference instance, denote the input prompt sequence as $S$. During the \textbf{initialization} phase, the input prompt $S$ undergoes a tokenization process $f_{\text{tokenization}}$, resulting in the tokenized representation $T = t_1 t_2 \ldots t_n$ as shown in \eqref{eq: tokenization}.

\begin{equation}
T = f_{\text{tokenization}}(S)
\label{eq: tokenization}
\end{equation}

After tokenization, the input $T$ passes through the embedding layer and gets converted to a multi-dimensional vector $E$, encoding the token's context and meaning. Then, the embedding $E$ is used to generate the query $E^Q$, cached $E^K$, and $E^V$ computed in formula \eqref{eq:query_vector} and \eqref{eq:key_value_vectors}.

\begin{equation}
E^Q = f^Q(E)
\label{eq:query_vector}
\end{equation}
\begin{equation}
E^K = f^Q(K) \quad ; \quad E^V = f^Q(V)
\label{eq:key_value_vectors}
\end{equation}

where $f^Q$, $f^K$, and $f^V$ represent multiplying with the weight matrices $W^Q$, $W^K$, and $W^V$.

During the \textbf{generation} phase, the current generated token $t_i$ is converted to a multi-dimensional vector $e_i$. The KV Cache is updated by appending $e_i^K$ to $K_{\text{cache}}^{i-1}$ and appending $e_i^V$ to $V_{\text{cache}}^{i-1}$ as shown in formula \eqref{eq:k_cache_update} and \eqref{eq:v_cache_update}.

\begin{equation}
K_{\text{cache}}^{i} \leftarrow \text{append}(K_{\text{cache}}^{i-1}, e_i^K)
\label{eq:k_cache_update}
\end{equation}
\begin{equation}
V_{\text{cache}}^{i} \leftarrow \text{append}(V_{\text{cache}}^{i-1}, e_i^V)
\label{eq:v_cache_update}
\end{equation}

The attention result is computed with the formula \eqref{eq:attention_formula}.

\begin{equation}
\text{Attn}(e_i^Q, K_{\text{cache}}^i, V_{\text{cache}}^i) = \text{softmax}\left(\frac{e_i^Q(K_{\text{cache}}^i)^T}{\sqrt{d}}\right)V_{\text{cache}}^i
\label{eq:attention_formula}
\end{equation}

While offering substantial computational advantages, KV caching requires an increased allocation of CPU memory to accommodate the storage requirements for the Key and Value matrices.


Specifically, in PQ, a high-dimensional vector $x$ is split into m distinct sub-vectors with non-overlapping dimensions $x = (x^0,…, x^{m-1})$, and each sub-vector $x^j$ is quantized by a sub-quantizer $q^j$ to the closest centroid $c^j_{i_j}$ from the sub-quantizer's codebook $C_j$: 
\begin{equation}
\text{pq}(x) = (q^0(x^0),...,q^{m-1}(x^{m-1})) = (c^0_{i_0},...,c^{m-1}_{i_{m-1}})
\end{equation}
The product-quantized representation of a vector is then converted into a sequence of codes representing the indexes of the corresponding centroids, and the original floating-point representation is discarded to achieve compression:
\begin{equation}
\text{enc}(x) = (i_0,...,i_{m-1}) \text{ where } \text{pq}(x) = (c^0_{i_0},...,c^{m-1}_{i_{m-1}})
\end{equation}
Using codebooks of $k$ centroids for each quantizer, PQ can compress vector $x$ into $m{\lceil}log_2 k{\rceil}$ bits.

For querying, PQ leverages Asymmetric Distance Computation (ADC). ADC computes distances between uncompressed query vectors and base vectors compressed into PQ codes, whereas symmetric computation finds the distances between compressed, PQ code representations of both the query and base vectors. ADC is more accurate than the symmetric counterpart while sacrificing a negligible amount of compression\cite{pq}.

To reduce distance computations and provide significant speedup, ADC utilizes lookup tables \cite{andre2017accelerated}. A query $q$ is split into m distinct sub-vectors $q = (q^0,…, q^{m-1})$, and a lookup table $D^j$ is calculated for each sub-vector $q_j$ which comprises the partial distances between $q_j$ and all centroids of the codebook $C_j$: 
\begin{equation}
D^j = (\lVert q^j-C^j[0]\rVert^2,...,\rVert q^j-C^j[k-1]\lVert^2)
\end{equation}
During querying, the distance between query vector q and PQ code representation of base vector c is found by summing the partial distances of the query sub-vectors of centroids associated with the PQ code according to the lookup tables.
\begin{equation}
\text{adc}(q, c) = \sum_{j=0}^{m-1} D^j[c[j]]
\end{equation}
Since only distance calculations are done when constructing the lookup table, speedup is greatly increased, particularly when querying large vector datasets.

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via OpenReview\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review (they are not required to look at more than the first $8$ pages of the submitted document).

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2024 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
\cref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
\cref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Theorems and such}
The preferred way is to number definitions, propositions, lemmas, etc. consecutively, within sections, as shown below.
\begin{definition}
\label{def:inj}
A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
If $f$ is injective mapping a set $X$ to another set $Y$, 
the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof} 
Left as an exercise to the reader. 
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
\label{lem:usefullemma}
For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is injective.
\end{lemma}
\begin{theorem}
\label{thm:bigtheorem}
If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
If $f:X\to Y$ is bijective, 
the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
The set $X$ is finite.
\label{ass:xfinite}
\end{assumption}
\begin{remark}
According to some, it is only the finite case (cf. \cref{ass:xfinite}) that is interesting.
\end{remark}
%restatable

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2024.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to \cref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent, e.g. use the actual current name of authors.
If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\section*{Accessibility}
Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the OpenReview reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
\nocite{langley00}


\subsection{Lookup-based Attention}

For a single attention head, the computation of attention scores for the $t$-th token is composed of $t$ dot product calculations between the current query embedding and previous key embeddings. dot product computations is dependent on the multiply-add (MAD) kernel, which is inefficient on CPUs due to the limited number of cores. In order to speed up attention score computations on CPUs, the reliance on MAD kernel needs to be removed. Therefore, we propose a new paradigm for computing attention called NoMAD (\underline{No} \underline{M}ultiply-\underline{AD}ds), which removes its reliance on MAD kernel by leveraging ultra low-latency (1-2 CPU cycles) in-register lookups. We primarily leverage four techniques to achieve lookup-based computations of attention: \begin{enumerate*}
    \item asymmetric attention score computations via product quantization,
    \item compressing dot product lookup tables to fit in SIMD registers,
    \item storing product-quantized key codes in a transposed blocked format cache,
    \item independent codebook learning per attention-head.
\end{enumerate*}

\subsection{Efficient Attention via Product Quantization}

Therefore, we leverage PQ to compute approximate dot products for attention. Specifically, we transform attention keys into product-quantized codes and only store codes in the key cache. For any query, we compute its dot products with respect to all centroids and store them in an LUT for each sub-quantizer. Then, the query-key dot product is computed through retrieving and accumulating the corresponding dot product from the LUT using key codes. This process mostly eliminates the use of MAD kernels in attention score computations, except the computation of LUT entries which is computationally lightweight compared to LUT lookups. However, this approach does not speed up attention, since a high proportion of the CPU cycles are wasted due to stalling and waiting for cache accesses to the LUT to complete. In order to achieve speedup, careful designs are required to avoid accessing slower units in the CPU memory hierarchy. In particular, we leverage two techniques to bypass cache accesses: fitting the LUT in registers and storing the key cache in a transposed blocked format.

% Previous works have shown that LLMs are robust to approximations of attention. For example, \citet{dejavu} demonstrates that LLM empirically follows the contextual sparsity hypothesis. Therefore, we leverage product quantization to transform attention score computations from dot products into lookups. Product quantization enables asymmetric lookups of dot products. Given a query vector $q$ and key vectors $k_1, \dots, k_t$, we are interested in computing the dot products between them. Each key is quantized to codes by finding the nearest centroid (in terms of L2 distance) in the codebook of each sub-quantizer. $S$ sub-quantizer produces $S$ codes. Then, the dot products between the segment of $\pi_s(q)$ with all centroids in the codebook is computed for all $s \in 1, \dots, S$ and stored in a lookup table (LUT). The codes of the keys are used to retrieve approximate dot products from the LUT.


\subsection{Fitting Lookup Table in Registers}

% Depending on the data storage unit, the speed of data retrieval by CPU can vary drastically. A lower level down in the CPU memory hierarchy is one to two orders of magnitude slower than the last level. 
In PQ, the number of times the CPU retrieves from LUT scales with the number of key vectors, hence can be significantly bottlenecked by the access speed to the LUT. 


\subsection{Transposed Blocked Key-code Cache}


\subsection{Attention Scores Through In-register Lookups}

The careful designs of register-resident LUT and key cache layout format enable computations of attention score through in-register lookups.  Similar to key caching in attention, in NoMAD-Attention, the PQ codes for the key embedding of the current token are computed by finding the centroid that minimizes L2 distance to the key, and inserted into the key-code cache.

% It serves two purposes: enable the use of SIMD instructions to perform batch lookups, achieve efficient storage of key codes.

% In NoMAD, the key cache does not hold the floating-point representation of keys, and instead stores the product-quantized key codes in a transposed blocked format. Figure \ref{fig:nomad_attn} presents a comparison of attention key cache and NoMAD key-code cache. The key code of each sub-quantizer uses 4 bits to represent 16 centroids in a codebook, and packed tightly (2 in a byte) to achieve storage efficiency. The PQ codes of a key is stored vertically in a column in a transposed manner, with 32 keys as a block. This facilitates the use of SIMD instruction for batch lookups (shuffles). The first 16 and the last 16 keys of a block is stored in an alternating manner, in order to maximize storage efficiency. The first 16 keys are obtained by using SIMD bit shifts, and the last 16 keys are obtained by using bit masking. After loading the LUT into registers, two SIMD shuffle instructions are issued to look up the first 16 keys and the last 16 keys.

% The layout allows using SIMD instructions to 

% The key codes are the indices, the LUT is the dictionary. Use the indices to retrieve the values of LUT. 


\subsection{Product Quantization}

Product Quantization (PQ) \cite{pq} is a method for compressing high-dimensional vectors to enable efficient nearest-neighbor search. PQ quantizes a floating-point vector into discrete codes. Traditional quantization approaches learn a set of clusters and quantize the vector to its nearest cluster centroid. PQ is based on the insight that a large number of centroids (e.g. $2^{128}$ centroids for 128-bit codes) are required to minimize quantization error for high-dimensional vectors, which is also computationally infeasible to learn or store. Therefore, PQ makes use of \textit{sub-quantizers}. for a $d$-dimensional vector space, a vector is divided evenly in dimension into $S$ segments. In each segment, the sub-vector has dimension $d_\mathrm{sub} = \frac dS$, and each sub-vector space is quantized independently. We use $\pi_s(e)$, where $s\in \{1\dots S\}$, to denote the function that maps a $d$-dimensional vector $e$ to its $d_\mathrm{sub}$-dimensional sub-vector of the $s$-th sub-quantizer.

\textbf{Learning Codebooks} A \textit{codebook} stores the set of cluster centroids for a sub-quantizer. In PQ, distinct codebooks are learned independently for each sub-quantizer. Given a set of vectors for learning, a clustering algorithm is used to partition each set of sub-vectors into a pre-determined number of clusters, each with a distinct centroid. The centroids are assigned a unique index and stored in the codebook. We use $b_{s,c}$ to denote the $c$-th centroid in the codebook of the $s$-th sub-quantizer. For a given vector $e$, the product-quantized codes of $e$, denoted $c_1, \dots, c_S$, are the indexes of the nearest centroid of each sub-quantizer, i.e.,

\begin{align}
    \mathrm{PQ}(e) =
    % \begin{bmatrix}
    %     c_1 & \dots & c_S
    % \end{bmatrix}
    [c_1 \dots c_S],
    \text{where } c_s = \argmin_c \big\lVert \pi_s(v) - b_{s, c}\big\rVert
\end{align}

The codes of product-quantized vectors are stored, and the original floating-point representation of the vector is discarded to achieve compression. Using $S$ sub-quantizers and $C$ centroids for each sub-quantizer, the product-quantized representation of a vector can be stored in $S\lceil\log_2C\rceil$ bits, where $\lceil x \rceil$ represents the ceiling function, rounding up to the nearest integer.


\textbf{Distance Computation via Lookups} PQ leverages Asymmetric Distance Computation (ADC) to reduce quantization errors in computed distances. To compute the distances between a query vector and a set of product-quantized base vectors, the distances between the non-quantized query vector and all centroids are first evaluated for each sub-quantizer and stored in a lookup table (LUT). Then, the PQ codes of the base vectors are used to retrieve the corresponding distances in the LUT. For each base vector, the retrieved distances are accumulated for all sub-quantizers to produce the final asymmetric distance to the query vector. Specifically, denoting the distance between query $q$ and the $c$-th centroid for the $s$-th sub-quantizer using $\mathrm{LUT}_s[c] = \mathrm{dist}\big(\pi_s(q), b_{s,c}\big)$, then the estimated distance between query $q$ and a product-quantized base vector $e$, where $
    \mathrm{PQ}(e) = [c_1 \dots c_S]$, is

\begin{equation}
    \widetilde{\mathrm{dist}}(q, e) = \sum_{s=1}^S \mathrm{LUT}_s[c_s]
\end{equation}

Different from traditional arithmetic distance computations, PQ distance evaluations primarily rely on repeated lookups from LUTs, hence achieving better efficiency by avoiding multiply-add operations.

% Instead of directly quantizing a vector to its nearest centroids, which is computationally infeasible 


% LLMs maintain model quality with negligible degradation in perplexity compared to the original model at $8\times$ key cache compression / 4 bits per float in key / $d_\mathrm{sub}=1$. Dimensionality reduction-based PCA-Attention leads to significant model quality degradation even at $2\times$ key cache compression.}

For the LLaMA-2-7B LLM, the original model achieves a perplexity of 8.615 and 8.756 under 16-bit weight and 4-bit quantized weight for the PTB dataset, while the NoMAD-Attention-based LLM with $8 \times$ key cache compression achieved 8.842 and 9.018 perplexity. On the WikiText-2 dataset, the original model achieves a perplexity of 5.796 and 5.963, whereas the NoMAD-Attention-based LLM achieved 5.993 and 6.185 perplexity.

As for the StableLM-3B-4E1T LLM, the original model achieves a perplexity of 11.977 and 16.119 under 16-bit weight and 4-bit quantized weight for the PTB dataset, whereas the NoMAD-Attention-based LLM with $8 \times$ key cache compression achieved 12.375 and 16.206 perplexity. On the WikiText-2 dataset, the original model achieves a perplexity of 9.231 and 12.599, whereas the NoMAD-Attention-based LLM achieved 9.638 and 13.111 perplexity.

It is also worth noting that $16 \times$ key cache compression also achieved decent perplexity under the two different LLMs running two different datasets.

\subsection{LLM Efficiency}

The results of the model efficiency comparison are depicted in Figure \ref{fig:efficiency}.

Concerning the time to finish prompt processing, the NoMAD attention-based CodeLlama-7B requires approximately $2.1 \times 10^6$ and $1.8 \times 10^6$ ms for models with 16-bit and 4-bit quantized weights, respectively. In comparison, the original model takes $3.0 \times 10^6$ and $2.8 \times 10^6$ ms, achieving a $1.5 \times$ increase at a 16k prompt length.

Regarding the decoding time for each token, the NoMAD attention-based CodeLlama-7B only takes about $450$ and $250$ ms for models with 16-bit and 4-bit quantized weights, respectively, while the original model takes $780$ and $500$ ms. This results in nearly a $2 \times$ increase at a 16k context length.

In terms of throughput measured by tokens per second, at the context length of 16k, the NoMAD attention-based CodeLlama-7B can achieve speeds of $4$ and $2.2$ tokens per second on models with 16-bit and 4-bit quantized weights, respectively. In contrast, the original model only manages $2$ and $0.8$ tokens per second, demonstrating more than a $2 \times$ increase at the 16k context length.

Overall, the NoMAD-Attention-based CodeLlama-7B (4-bit quantized weights) achieves a $2\times$ speedup over the original CodeLlama-7B (4-bit quantized weights) at relatively long prompt and context length (e.g. 16k).

The results of the Attention efficiency comparison are illustrated in Figure \ref{fig:ablation}.

For the standard reference, regular Attention exhibits an Attention score latency of approximately 580 $\mu$s and a key caching latency of around 3.0 $\mu$s. In comparison, conventional PQ-Attention (8-bit code, $d_\mathrm{sub}=2$) demonstrates a limited speedup in Attention score latency (470 $\mu$s) and a significantly longer key caching latency of more than 15 $\mu$s. On the other hand, NoMAD-Attention (4-bit code, $d_\mathrm{sub}=1$) markedly reduces the latency of Attention score computation for 16k queries at 16k context length, with only less than 80 $\mu$s—achieving over a $5 \times$ speedup. It also exhibits a decent key caching overhead, taking only half the time of normal PQ-Attention.
